Cross-Lingual and Cross-Cultural Variation in Image Descriptions

Do speakers of different languages talk differently about what they see? Behavioural and cognitive studies report cultural effects on perception; however, these are mostly limited in scope and hard to replicate. In this work, we conduct the first large-scale empirical study of cross-lingual variation in image descriptions. Using a multimodal dataset with 31 languages and images from diverse locations, we develop a method to accurately identify entities mentioned in captions and present in the images, then measure how they vary across languages. Our analysis reveals that pairs of languages that are geographically or genetically closer tend to mention the same entities more frequently. We also identify entity categories whose saliency is universally high (such as animate beings), low (clothing accessories) or displaying high variance across languages (landscape). In a case study, we measure the differences in a specific language pair (e.g., Japanese mentions clothing far more frequently than English). Furthermore, our method corroborates previous small-scale studies, including 1) Rosch et al. (1976)'s theory of basic-level categories, demonstrating a preference for entities that are neither too generic nor too specific, and 2) Miyamoto et al. (2006)'s hypothesis that environments afford patterns of perception, such as entity counts. Overall, our work reveals the presence of both universal and culture-specific patterns in entity mentions.

==> sections/literature_review.tex <==
Our study falls under the umbrella of works that study cultural effects on visual tasks. Early studies used small-scale, controlled experiments, while the recent rise in amount of publicly available visual data with human annotations has prompted large-scale and less controlled studies exploiting computational methods to investigate these large-scale corpora.

\subsection{Small-Scale Controlled Studies}

\paragraph{Color discrimination.}
\citet{winawer2007russian} test English and Russian speakers in a speed color discrimination task, where the colors are selected from a spectrum around the blue color, to which English speakers have a single word while Russian speakers separate lighter blue (\emph{goluboy}) and darker blue (\emph{siniy}). Russian speakers showed improved speed in discriminating two colors when one was light blue and the other dark, while English speakers did not show a similar effect.
\citet{mitterer2009influence} presented discs on a yellow-to-orange spectrum to German and Dutch speakers, and asked them to classify the discs to yellow or orange. The discs were located at the middle light of a traffic light; while the standard color for the middle light in both Germany and the Netherlands, the words use to describe these colors differ: \emph{gelb}, i.e. yellow for German and \emph{oranje}, i.e. orange for Dutch. Consistently, Dutch speakers were more likely to classify the colors as Orange, even though the same stimulus was shown to the two groups.

\paragraph{Visual illusions.}
\citet{segall1963cultural} show participants geometric illusions (e.g., two lines of equal length terminated with fins protruding either inward or outward, where participants tend to judge the line with outward fins as longer) and find cross-cultural difference in the number of illusion responses.

\citet{caparos2012exposure} show participants from a traditional village population and from an urban population two visual illusions (the Ebbinghaus illusion and a local/global focus task), and show that participants from the traditional population demonstrate a local bias.

\citet{linnell2018urban} study lightness contrast illusions: a gray circle would appear darker on a white background compared to a black background. When non-urban dwelling participants were presented with the illusion, they showed significantly higher contrast than urban dwelling participants.

\paragraph{Difference in reading facial expressions.}
\citet{jack2009cultural} show that Eastern participants tend to focus on the eyes alone while reading facial expressions, while Western participants scan the entire face.

\paragraph{Difference in environments}
\citet{miyamoto2006culture} study the difference in typical environments encountered by different cultures, and the effects these differences have on perception.
The authors first compute the number of objects in photos taken in Japan and the United States, and show that photos taken in Japan contains more objects using both subjective (human annotator counts) and objective (automated algorithm count) measures. Next, they show that Japanese participants were more likely then American participants to identify a change in an object not in the center of the image, and both Japanese and Americans were more likely to identify a change in an object not in the center of the image if the image was taken in Japan.

\paragraph{Difference in contextual attention.}
\citet{masuda2001attending} show animated clips of underwater scenes to Japanese and Americans and subsequently collected their description of the scenes. The Japanese participants made more statements about contextual information and relationships. \citet{senzaki2014perception} replicate this result for Canadian and Japanese, while \citet{senzaki2016communication} show that the effect is higher for adult participants compared to children.

\subsection{Large-Scale Studies}
Several previous studies have recognized the advantage of utilizing existing public image-caption datasets as a test bed for large-scale experiments of cultural effects on language generation.

\citet{van-miltenburg-etal-2017-cross} compare descriptions generated by English, German and Dutch annotators on images taken from Flickr30k~\cite{young2014image}. They study lexical aspects such as the use of negation words, as well as the degree of specificity in annotations across languages, i.e., do annotators provide the name or a general description for locations and objects. Their approach diverges from ours in several key respects. First, we focus on the XM3600 corpus that contains cross-cultural images. Second, we study a wider range of languages. Finally, we systematically study patterns of object selection by developing tools for object mention identification, whereas their methodology involves manual analysis of specific images to gain insights regarding specificity. 

Most similar to our work, \citet{ye2023cultural} use XM3600 to study cultural differences in perception. The authors translate captions to English and then use models to generate scene graphs, and compare objects, relations and attributes across 7 languages. While also comparing mentions of objects across languages, they differ in their motivation, and therefore in their experimental setup as well. First, they only show that captions from different languages mention different objects, while we study this differences in depth; Second, they focus on 7 languages while we focus on all 36 languages of XM3600.

\citet{ventura2023navigating}

\subsection{WordNet}

WordNet~\cite{miller1995wordnet} is a large database of English phrases, including meaning of phrases and relations between phrases. WordNet defines a tree structure of synsets, where each synset represents one meaning of an English word, e.g., the synset \emph{bank.n.01} represents the \emph{river bank} meaning of the word `bank' and is the direct child of the \emph{slope.n.01} synset, while the synset \emph{bank.n.02} represents the \emph{financial institution bank} meaning and is the direct child of the \emph{financial\_institution.n.01} synset.

==> sections/old_04_experiments.tex <==
In this section we experiment on our entity mentions corpus, extracted from XM3600 captions.

\subsection{Definitions}
Each example in XM3600 associates an image with multiple captions in each language $l \in \mathcal{L}$: $\mathcal{D}_l = \{i, \{c_j\}_{j=1}^n\}_{i=1}^{3600}$.
For a given entity $o \in \mathcal{O}$ (i.e., WordNet synset) and caption (a sequence of words) $c \in \mathcal{V}^+$, we define the function $f(o, c)$ as returning 1 if $o$ is in the list of entities extracted from $c$, and 0 otherwise.
If a synset is extracted for a given caption, all its ancestors in the WordNet tree are also considered extracted.

\paragraph{Entity saliency.}

We define the saliency of entity $o$ in image $i$ as the fraction of captions of this image for which $o$ is in the list of extracted entities.
Formally, given
% Note: since we use WordNet synsets as a proxy for entity types, we exploit the tree structure of WordNet so that if a synset was extracted for a given caption, all its ancestors in the tree are also considered as extracted in this caption.
captions for $i$ in multiple languages
$\mathcal{L}_1, ..., \mathcal{L}_m$,
\begin{equation*}
    \begin{matrix}
    c^{\mathcal{L}_1}_{1}, & c^{\mathcal{L}_1}_{2}, & ..., & c^{\mathcal{L}_1}_{n_1} \\
    c^{\mathcal{L}_2}_{1}, & c^{\mathcal{L}_2}_{2}, &..., &c^{\mathcal{L}_2}_{n_2} \\
    ..., & ..., & ... & ... \\
    c^{\mathcal{L}_m}_{1}, & c^{\mathcal{L}_m}_{2}, &..., &c^{\mathcal{L}_m}_{n_m}
    \end{matrix}
\end{equation*}
we denote the saliency of $o$ in $i$ for captions in language $l \in \mathcal{L}$ as
\begin{equation} \label{eq:ls_saliency}
    \text{saliency}(l, o, i) = \frac{\sum_{j=1}^{n_l}{f(o, c^{l}_{j})}}{n_l}
\end{equation}
See Figure~\ref{fig:image_example} for an example. Composing the saliency scores across entities, languages, and images, we obtain a tensor of size $M \in [0, 1]^{|\mathcal{L}|, |\mathcal{O}|, |\mathcal{I}|}$. The cell $M_{l, o, i}$ represents the saliency of entity $o$ in language $l$ for image $i$.

\subsection{Geographic and Genetic Effects} \label{sec:typology_saliency_corr}

We first study whether languages that are geographically close, genetically related, or typologically similar, also share similar patterns in terms of entity saliency. To this end, we correlate two distance metrics: typological distance and saliency distance between languages.

\paragraph{Typological distance.}
We use \texttt{lang2vec}~\cite{littell2017uriel} to source pre-computed geographical, genetic and featural distances between languages.

\paragraph{Saliency distance.}
We define the saliency distance between two languages $(\mathcal{L}_l, \mathcal{L}_k)$ as follows.
Given the tensor of saliency scores $M$ obtained from Equation~\ref{eq:ls_saliency}, 
we measure saliency distance as the Euclidean distance between language-specific scores: $\sqrt{\sum_o^{|\mathcal{O}|} \sum_i^ {|\mathcal{I}|}[(M_{\mathcal{L}_l, o, i}) - (M_{\mathcal{L}_k, o, i})]^2}$

\input{tables_and_figures/typology_saliency_correlation}

\paragraph{Correlation significance test.}
For each distance metric, we construct a distance matrix where the $(l, k)$ cell represents the distance between $\mathcal{L}_l$ and $\mathcal{L}_k$ according to that metric.
We use the Mantel test~\cite{mantel1967detection} to compute the correlation between the saliency distance matrix and each of the typological distance matrices. Results are presented in Table~\ref{tab:mantel}. We find that saliency distance correlates weakly with both geographic and genetic distances based on $r \in [-1, 1]$ scores, but $p$-values are statistically significant. On the other hand, we find no significant correlation with featural distance.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{tables_and_figures/violin_saliency_variation}
    \caption{Violin plot of the distribution of saliency scores across languages for each entity category. Saliency scores are averaged across all images containing the entity. Silver lines indicate quartiles.}
    \label{fig:violin_saliency_variation}
\end{figure*}

\subsection{Cross-lingual Variation of Entity Saliency} \label{sec:cross_lingual_var}
Next, we investigate which entity categories exhibit cross-lingual variation in saliency. In other words, which entities are universally salient or non-salient? The saliency of which ones varies the most across languages?

Let $\mathcal{I}_o \subseteq \mathcal{I}$ identify the subset of images where entity $o$ is visible according to our manual image annotation mentioned in Section~\ref{sec:synset_filtering}. Then we calculate the global saliency of an 
entity $o$ and language $l$ as the mean saliency across images $i \in \mathcal{I}_o$.
% To ensure our sample is sufficient for meaningful results, we only include synsets instantiated in at least 100 images in this analysis, i.e. $|\mathcal{I}_o| \ge 100$, reducing the original 25 root synsets to 15.

We plot the resulting global saliency scores in Figure~\ref{fig:violin_saliency_variation}: for each entity category, we report their distribution across languages.
First, we find that certain entities are universally salient: for instance, \textsc{animal.n.01} (0.693), \textsc{food.n.01} (0.669), and \textsc{person.n.01} (0.660). Remarkably, these include the only two entities with animacy \citep{dahl2000animacy}. Conversely, we found that some entities are universally non-salient, e.g., \textsc{bag.n.01} (0.109), \textsc{timepiece.n.01} (0.093), and
\textsc{jewelry.n.01} (0.070). These broadly fall into fashion accessories and apparel.

Finally, Figure~\ref{fig:violin_saliency_variation} lets us identify entities whose global saliency exhibits the highest standard deviation across languages, i.e., \textsc{sky.n.01} (0.109), \textsc{plant.n.02} (0.069), \textsc{mountain.n.01} (0.063).
This suggests that the inclusion of entities commonly located in the background in the descriptions varies between languages, consistent with findings from previous small-scale, controlled studies~\citep[e.g.,][]{miyamoto2006culture}.

\subsection{Case Study: English versus Japanese} \label{sec:en_ja_saliency}
While the results in Section~\ref{sec:cross_lingual_var} inform us of global cross-linguistic tendencies, a finer-grained analysis could try to determine the differences in saliency between specific pairs of languages.
Nevertheless, this raises the concern that the data collected for XM3600 may be insufficient, as it employed only two annotators per language.
Thus, any observed effect would reflect the preferences of those individuals rather than a broader trend.

To mitigate this potential drawback, we focus on a case study for a language pair, namely English--Japanese, for which a significantly larger parallel image captioning dataset is available.
Specifically, the MSCOCO~\cite{lin2014microsoft} dataset comprises a substantial collection of English image captions, encompassing approximately 120K images, each accompanied by an average of five captions. STAIR-captions~\cite{yoshikawa2017stair} is a Japanese version of MSCOCO, wherein Japanese annotators have provided original captions, without resorting to translation, for each image, yielding five captions per image. Overall, about 2100 annotators contributed to the STAIR-captions dataset.

Similarly to Section~\ref{sec:cross_lingual_var}, we define the global saliency for a specific entity category in each language as the mean saliency across all images in MSCOCO in the captions for that language.
For each root synset, we calculate the ratio between the English and Japanese per-language saliency. Table~\ref{tab:en_ja_saliency} plots the top five root synsets in terms of saliency ratio, in both directions.
While we only report results for MSCOCO due to the small sample size of XM3600, we do note that similar rankings were found with XM3600, where the synsets with the highest saliency ratios between Japanese and English were \textsc{clothing.n.01} (3.78) and \textsc{body\_part.n.01} (3.52).
As expected, the concepts where we record the highest differences between Japanese and English are also among those with the least saliency cross-linguistically, as they lie at the bottom of Figure~\ref{fig:violin_saliency_variation}.

\input{tables_and_figures/en_ja_saliency}

\paragraph{Statistical significance.}
To assess statistical significance, we conduct a comparison between the lists of global saliency values associated with each synset in the two languages.
We use the Wilcoxon signed-ranked test~\cite{wilcoxon1992individual} with Bonferroni correction. All entities in Table~\ref{tab:en_ja_saliency} except \textsc{musical\_instrument.n.01} show significance.

% \begin{figure} [t]
%     \centering
%     \includegraphics[width=\columnwidth]{tables_and_figures/shirt_examples_coco2.png}
%     \caption{An image for which all Japanese annotators and none of the English annotators mentioned shirts. Image and captions are taken from MSCOCO and STAIR-captions (we select the first two captions).}
%     \label{fig:shirt_coco}
% \end{figure}

\paragraph{Qualitative Analysis: Clothing.}
We now zoom in further onto a specific category, showcasing how our method can serve as an exploration tool for identifying preliminary findings that can later be validated through controlled experiments.
We focus on clothing-related entities, which showed the highest saliency ratio between Japanese and English.
To gain deeper insights into the origin of this disparity, we conduct the statistical significance test for all the explicit synsets that are descendants (see Section~\ref{sec:synset_selection}) of the \textsc{clothing.n.01} synset. We find that only the \textsc{shirt.n.01} synset was significantly more salient in Japanese in both MSCOCO and XM3600.
This indicates that differences in high-level categories may be driven by specific (culturally motivated) entities.

%EDO: This is nice but maybe leave out for now (to be included if we have extra page for CR)
%Next, we manually review images where all Japanese annotators identified shirts, but none of the English annotators did (11 images in MSCOCO, 20 in XM3600). Interestingly, in both datasets, there were no cases where all English annotators identified shirts while none of the Japanese annotators did.

% \begin{figure*} [tb]
%     \centering
%     \includegraphics[width=\textwidth]{tables_and_figures/shirt_examples_xm3600.pdf}
%     \caption{Examples of images for which all Japanese annotators and none of the English annotators mentioned shirts. Images and captions taken from XM3600.}
%     \label{fig:shirt_xm3600}
% \end{figure*}

%We observe a consistent trend among the Japanese annotators wherein they mention the color of the shirts depicted in the image.\footnote{This raises the suspicion that the observed disparity may be attributable to a particular annotation guideline within STAIR-captions pertaining to colors or attributes; however, no such guideline was provided in STAIR-captions. For the full annotation guidelines for all datasets see Appendix~\ref{sec:app_annotation_guidelines}.} An example image and captions are shown in Figure~\ref{fig:shirt_coco}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{tables_and_figures/depths_dist2.pdf}
    \caption{Distribution of depths in the WordNet synset hierarchy across languages.}
    \label{fig:depths_dist}
\end{figure}

\begin{figure*} [t]
    \centering
    
    \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=\columnwidth]{tables_and_figures/object_num}
    \caption{Home vs Abroad}
    \label{fig:object_num_home_abroad}
    \end{subfigure}%
    \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=\columnwidth]{tables_and_figures/object_num_enja}
    \caption{Japanese- vs English-speaking zones}
    \label{fig:object_num_enja}
    \end{subfigure}
    \caption{Average number of entities mentioned by speakers of 31 languages in captions of images captured in different locations. The dashed line indicates identity.}
    \vspace{11pt}
\end{figure*}

\subsection{Granularity} \label{sec:granularity}

% In this section we study the granularity of object that different languages choose to describe.
Given a hierarchy of categories and their corresponding nominal expressions, from the most generic to the most specific, the level chosen for describing entities is in principle arbitrary. For instance, when describing an image of an armchair, annotators can choose to label it as \textit{furniture}, \textit{chair} or \textit{armchair}, sorted by their depth in the hierarchy in descending order.
\citet{rosch1976basic} introduced the concept of \emph{basic level categories} which are the categories in a hierarchy preferred over more specific subordinates or broader superordinates. If indeed such basic levels exist for a specific language, we would expect the distribution of the levels of mentioned entities to form a two-tailed distribution, with the basic level being used more frequently than the very specific or very general concepts.

We use the depth in the WordNet tree as a proxy for the granularity of an entity category.
Figure~\ref{fig:depths_dist} plots a histogram of synset depths of entities mentioned in each language. Although the number of mentions varies across languages at different levels, all distributions are two-tailed with most mass concentrating in the centre (levels 5--10 in the WordNet hierarchy), in support of the basic-level category hypothesis.

\subsection{Entity Count} \label{sec:object_num}

Does the location of an image affect the number of entities mentioned in its descriptions, due to its familiarity or complexity of the environment? 
To answer this question, we use the location indicators provided for each image in XM3600, where 100 images per language were captured in regions where that language is spoken.
for each language, we first compare the average entity mentions for the 100 images from its relevant regions versus the other 3000 images from abroad.

Figure~\ref{fig:object_num_home_abroad} illustrates that most languages mention around the same number of entities regardless of familiarity, i.e., whether the image was taken at home or abroad. The correlation between these two numbers is strong, with Pearson's $\rho=0.64$, and significant, with $p<10^{-4}$. Major exceptions, however, are found in a group of languages including Filipino, Vietnamese, Japanese, and Thai, which resort to significantly more entities when describing images taken at home. Notably, these languages are spoken in (South) East Asia, suggesting a potential areal effect. %Vice versa, the Russian language is unique in mentioning much fewer entities in images taken in its area (-0.36).

In addition, we validate one of the studies of \citet{miyamoto2006culture}, namely that patterns of attention are (at least in part) afforded by different environments in images (e.g., Japan vs America). In particular, we compare the average number of entities mentioned in XM3600 pictures captured in Japanese- vs English-speaking zones. We show the results in Figure~\ref{fig:object_num_enja}. We find that Japanese images consistently elicited more entity mentions in all 31 languages (including both Japanese and English). This aligns with \citet{miyamoto2006culture}'s finding that speakers of both languages count more entities in Japanese images.

==> tables_and_figures/lang_clusters.tex <==
\begin{table}[!tb]
\centering
\begin{tabular}{cc}
\toprule
Cluster & Languages \\
\midrule
\multirow{3}{*}{1} & Czech, Danish, German, Greek, \\
 & Spanish, Finish, French, Croatian, \\
 & Hungarian, Italian, Dutch, Norwegian, \\
 & Polish, Portuguese, Swedish \\
\midrule
\multirow{2}{*}{2} & Indonesian, Japanese, Korean, \\
& Thai, Vietnamese, Chinese \\
\midrule
3 & Russian, Ukranian \\
\midrule
\multirow{2}{*}{4} & Arabic, English, Persian, Filipino, \\
& Hindi, Quechua, Swahili, Telugu \\
& Turkish \\
\midrule
5 & Hebrew, Romanian \\
\midrule
6 & Bengali \\
\midrule
7 & Maori \\
\bottomrule
\end{tabular}
\caption{The resulting clusters of spectral clustering of a weighted undirected graph where each node is a language and the weights are the similarities in class saliency.}
\label{tab:lang_clusters}
\end{table}

==> tables_and_figures/saliency_std.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{llll}
\toprule
Rank & Entity & $saliency\_std$ \\
\midrule
1 & Sky & 0.109 \\
2 & Plant & 0.069 \\
3 & Mountain & 0.064 \\
4 & Tableware & 0.054 \\
5 & Clothing & 0.054 \\
\midrule
11 & Bag & 0.026 \\
12 & Person & 0.026 \\
13 & Vehicle & 0.023 \\
14 & Food & 0.018 \\
15 & Animal & 0.017 \\
\bottomrule
    \end{tabular}
    \caption{Entity categories with high (top) and low (bottom) standard deviation of saliency across languages.}
    \label{tab:saliency_std}
\end{table}
